Looking for Clues of Language in Multilingual BERT to Improve Cross-lingual Generalization

Token embeddings in multilingual BERT (m-BERT) contain both language and semantic information. We find that the representation of a language can be obtained by simply averaging the embeddings of the tokens of the language. Given this language representation, we control the output languages of multilingual BERT by manipulating the token embeddings, thus achieving unsupervised token translation. We further propose a computationally cheap but effective approach to improve the cross-lingual ability of m-BERT based on this observation.

==> sections/conclusion-orig.tex <==
\section{Conclusion}
In this paper, we examined the existence of language-specific information in
m-BERT embeddings and succeeded in the task of unsupervised token translation
by manipulating language-specific information. 
The proposed methods are further shown to be effective in improving
cross-lingual embedding alignment and cross-lingual transfer learning.
We will further explore the proposed approach on more downstream tasks.


==> sections/intro-orig.tex <==
\section{Introduction}
Multilingual BERT (m-BERT) \cite{devlin:19} has already demonstrated its
extraordinary strength in cross-lingual transfer on a variety of
tasks~\citep{conneau:18, wu:19, hsu-etal:19, pires:19}, and this has been
credited to the cross-lingual alignment of its internal representations, which
is a phenomenon that semantically-similar or functionally-similar words from
different languages are represented with similar embeddings. %%幫cite

Although m-BERT does exceptionally well in aligning cross-lingual
representation, we believe the language information is still in token
embeddings.
One evidence is that m-BERT learns to reconstruct the same sentences as input,
so when masking one token from an English sentence, the probability of decoding
a Chinese token in that position is very low. 
Hence, m-BERT reserves some implicit language information in the embedding
space that can be disentangled from semantic information.
To verify the assumption, we show that if an English sentence is given to
m-BERT as input, and then its embeddings are shifted in a specific direction in
the embedding space, then m-BERT would output a sentence in another language
semantically close to the input sentence. 

After showing the existence of language information in the embeddings of
m-BERT, we eliminate these language-specific variations in the embeddings, and
demonstrate that its a practical way to boost zero-shot cross-lingual
transferability of m-BERT on downstream tasks.

In literature, there are studies trying to improve cross-lingual alignment in
pre-trained m-BERT. For example, \citet{Cao2020Multilingual} proposed to
finetune m-BERT on a small parallel data and \citet{libovick2020language}
proposed to unsupervisedly zero-centering the embeddings language by language
to achieve language neutrality and showed progress on retrieval tasks. Our work
is concurrent to \citet{libovick2020language}'s and has similarities in
approaches. But the approach here is more effective.  


The contributions of this work can be summarized as the following:
\begin{itemize}
  \item The language information in m-BERT can be represented by the average of
  all token embeddings of the specific language. This is verified by {\it
  unsupervised token translation}.
  \item The cross-lingual transferability of m-BERT in downstream tasks can be
  improved by manipulating token embeddings.
  \item We compared our method to other cross-lingual embedding alignment methods.
\end{itemize}





==> sections/methods-orig.tex <==
\section{Language Representation}
\label{section:methods}

We assumed that we have $n$ languages denoted by $\{L_1, L_2, \ldots, L_n\}$
and their corresponding corpora. 
%We first defined the following notations to describe our methods of extracting language representation.
%Then we show how to eliminate language information or add language information in m-BERT.


\paragraph{Context-Dependent Representation}
Given an input sequence $x$ and token index $i$, we denote the hidden
representation in layer $l$ by $\bm{h}^l_{x_i}$.

\paragraph{Mean of Language} 
Given a language $L$ and its corresponding corpora $C$ contain a set of
sentences $x$, we denote the mean of language of layer $l$ by
\[\vect{R}^l_{L}=\mathop{\Eb}_{x_i \in C}\left[\vect{h}^l_{x_i}\right],\]
which represents the mean of all the token embeddings in the corpora.
We assume that mean of language contains language-specific information but no
semantic information.

Although the assumption about language representation here seems naive, in the
experiments, we show that $\vect{R}^l_{L}$ represents the language information
in token embeddings well.
For each language $L$, there is a language-specific representation
$\vect{R}^l_{L}$ for each layer $l$.
Because we do not know $\vect{R}^l_{L}$ from which layer $l$ represents
language $L$ the best, $l$ is a hyperparameter in the following algorithms.

\paragraph{Zero-mean} 
We can simply subtract each token embedding $\vect{h}^l_{x_i}$ by mean of
language $\vect{R}^l_{L_k}$ to eliminate language-specific information.
The subtraction moves the token embedding to a language-agnostic joint space.
The language-agnostic hidden representation $\hat{\vect{h}}^l_{x_i}$ can be
written as
\begin{equation}
    \hat{\vect{h}}^l_{x_i} = \vect{h}^l_{x_i} - \vect{R}^l_{L_k},
    \label{eq:zero}
\end{equation}
where $\vect{h}^l_{x_i}$ is extracted from the token $x_i$ in $L_k$.

\paragraph{Mean Difference Shift (MDS)}
\begin{CJK*}{UTF8}{gbsn}
Besides eliminating language information, we can move the embedding in the
space of $L_1$ to the space of $L_2$, or \textit{unsupervised token
translation}.
That is, given the embedding of \textit{me} in English, we can modify the
embedding to make it be interpreted by m-BERT as the embedding of 我
(\textit{me} in Chinese).
\end{CJK*}

We fed an $L_1$ sentence into m-BERT, extracted the embedding of each token at
layer $l$. 
Then we subtract the embedding by $\vect{R}^l_{L_1}$ as in (\ref{eq:zero}) to
remove the information of $L_1$, and then we add $\vect{R}^l_{L_2}$  to shift
the embedding to the space of $L_2$.
Formally, we modified token embedding $\vect{h}^l_{x_i}$ in $L1$ into embedding
$\tilde{\vect{h}}^l_{x_i}$ in $L2$ as below:
\begin{equation}
    \tilde{\vect{h}}^l_{x_i} = \vect{h}^l_{x_i} + \vect{R}^l_{L_2}-\vect{R}^l_{L_1}.
    \label{eq:MDS}
\end{equation}

%\[\tilde{\vect{h}}^l_{x_i} = \vect{h}^l_{x_i} + \vect{R}^l_{L_2}-\vect{R}^l_{L_1}.\]

% \paragraph{Mean Difference} Given two languages $L_1, L_2$, we defined the mean difference of layer $l$ as 
% \[\vect{D}^l_{L_1\veryshortarrow L_2}=\vect{R}^l_{L_2}-\vect{R}^l_{L_1}.\]

% For convenience, we consider 2 language case.

% We assume that token representations could be broken into language-neutral and language-specific components . Language-neutral components are related to semantics and we assume that semantics components are uniformly distributed for a language. 
%and language-specific component is the same for all tokens belonging to the same language. Hence the semantic information is eliminated in the mean of language but not language-specific representation.

% semantic embedding of a language is uniform distributed  in the embedding space, and language-specific information is the same in the language. Hence the semantic information is eliminated in the mean of language but not language-specific representation.

%\quad \text{if $\vect{h}^l_{x_i}$ is extracted from $L_k$.}


==> sections/retrieval-orig.tex <==
\input{sections/tables/tatoeba}
\input{sections/tables/bucc2018}

\section{Cross-lingual Sentence Retrieval}
Extracting parallel sentences from a comparable corpus between two languages is
one of the standard methods of evaluating cross-lingual
embeddings~\citep{hu2020xtreme, zweigenbaum-etal-2017-overview,
artetxe2018massively}. 
In this section, we demonstrated that embeddings shifted by MDS are better
cross-lingually aligned through evaluations on a sentence-level retrieval task.  

\subsection{Task}
We evaluated the effect of MDS and Zero-mean on two sentence retrieval tasks:
BUCC2018 and Tatoeba. 
We used the mean vector of all token embeddings in a sentence as the sentence
embedding and cosine similarity as distance metric. 
Token embeddings were extracted from a specific layer of BERT encoder, and MDS
or Zero-mean shifts pre-computed on the whole dataset were applied directly to
the extracted embeddings. 
% Accuracy was the evaluation metrics used for evaluation.

\subsection{MDS vs Zero-Mean}
\label{sec:mds_zm_diff}

Although applying MDS or applying Zero-mean in sentence retrieval task seem
very similar at first glance, they have subtle differences. 
Assume we have sentence embeddings $\vect{v}_1 \in L_1$ and $\vect{v}_2 \in
L_2$, and the two sentences in different languages have the same semantic
meaning.
Assume there exist \textit{real} language representations $\vect{R}_{L_1}^*$
and $\vect{R}_{L_2}^*$ that can perfectly eliminate language from
embedding\footnote{Unknown to us}, leading to
$\vect{v}_1-\vect{R}_{L_1}^*=\vect{v}_2-\vect{R}_{L_2}^*$.
The language representations $\vect{R}_{L_1}$ and $\vect{R}_{L_2}$ obtained by
average are the approximation of the real ones\footnote{The superscript $^l$ is
ignored here for simplicity}, and $\delta_1$ and $\delta_2$ are difference
between real and approximate language representations. 
\[
\begin{split}
	 &\vect{v}_1-\vect{R}_{L_1} \neq \vect{v}_2-\vect{R}_{L_2} \\
  \rightarrow& \vect{v}_1-\vect{R}_{L_1}-\vect{\delta}_1=\vect{v}_2-\vect{R}_{L_2}-\vect{\delta}_2
\end{split}
\]
Then the cosine similarities of $\vect{v}_1$ and $\vect{v}_2$ after Zero-mean
or MDS are shown as below,
\[
\small
\begin{split}
\cos_\text{MDS}\left(\vect{v}_1,\vect{v}_2\right)
&= \frac{ \left(\vect{v}_1-{\vect{R_{L_1}}}+\vect{R_{L_2}}\right) \cdot \vect{v}_2}
{\left\lvert\vect{v}_1-{\vect{R_{L_1}}}+\vect{R_{L_2}}\right\rvert\left\lvert\vect{v}_2\right\rvert}\\
&= \frac{ \left(\vect{v}_2+\vect{\delta}\right) \cdot \vect{v_2}}
{\left\lvert \vect{v}_2+\vect{\delta}\right\rvert\left\lvert\vect{v}_2\right\rvert}, \text{ where } \vect{\delta}=\vect{\delta}_1-\vect{\delta}_2\\\
\cos_\text{Zero-mean}\left(\vect{v}_1,\vect{v}_2\right)
&= \frac{ \left(\vect{v}_1-{\vect{R_{L_1}}}\right) \cdot \left(\vect{v}_2 -{\vect{R_{L_2}} }\right)}
{\left\lvert\vect{v}_1-{\vect{R_{L_1}}}\right\rvert\left\lvert\vect{v}_2-{\vect{R_{L_2}}}\right\rvert}\\
&= \frac{
\left(\vect{v}_2- \vect{R^*_{L_2}} + \vect{\delta}_1\right) \left(\vect{v}_2- \vect{R^*_{L_2}} + \vect{\delta}_2\right)}
{\left\lvert\vect{v}_2- \vect{R^*_{L_2}} + \vect{\delta}_1\right\rvert \left\lvert\vect{v}_2- \vect{R^*_{L_2}} + \vect{\delta}_2\right\rvert}\\
\end{split}
\]
The above result shows that Zero-mean method is more sensitive to the
approximate error when $\left\lvert\vect{v}_2 \right\rvert >
\left\lvert\vect{v}_2- \vect{R_{L_2}}\right\rvert >
\max\left(\abs{\vect{\delta_1},\abs{\vect{\delta_2}},\abs{\vect{\delta}}}\right)$.\footnote{This
is very possible. Because $\vect{v}_2$ is in $L_2$, it may has the same
direction as $\vect{R}_{L_2}$.}
The differences between the two methods were further verified in the experiments.

%for cosine similarity is shown in Appendix~\ref{sec:mds_zm_diff}. 

%$\left\lvert\vect{v_2} \right\rvert > \left\lvert\vect{v_2}- \vect{R_{L_2}}\right\rvert > \max\left(\abs{\vect{\delta_1}}, \abs{\vect{\delta_2}}, \abs{\vect{\delta}}\right)\geq 0$.


\subsection{Result}
\input{sections/tables/pos}
\input{sections/tables/dep}
Results of sentence retrieval were shown as table~\ref{tab:bucc2018} and
table~\ref{tab:tatoeba}. 
On BUCC2018 dev-set and test-set, embeddings shifted by MDS consistently
achieved higher accuracies on all of the languages, and Zero-meaned embeddings
were worse than doing nothing. 
On the Tatoeba test-set, the MDS embeddings
were also the best in most of the languages
except for Hindi, Russian and Vietnamese.


%On the other hand, although MDS and Zero-mean both improved contextualized word retrieval performance over original representations, but Zero-mean was consistently better than MDS on all of the languages. In contrast, applying MUSE was even worse than using original representations.   







==> sections/tables/decoding.tex <==
7

de	0.0009816792772924603	8.729020966410274e-05	5.88926574225684e-158
el	0.000528838196795067	6.824208183147285e-06	5.505280940170566e-159
fr	0.001161229788479343	2.811500561991077e-05	1.9353432760567704e-158
zh	4.843513871164543e-05	2.9489744885308178e-05	2.5448779731929048e-158

11
de	0.0009823340923527364	8.729020966410274e-05	5.88926574225684e-158
el	0.0005605474824528539	1.9504863606635106e-05	1.6117553999272969e-158
fr	0.0011606190149224178	2.811500561991077e-05	1.9353432760567704e-158
zh	5.2328933053128505e-05	3.42256372247982e-05	3.0024491766597042e-158


12

de	0.0009959576389104146	8.729020966410274e-05	5.88926574225684e-158
el	0.000549174372923765	1.929566329833045e-05	1.603091291521212e-158
fr	0.001175660701883424	2.811500561991077e-05	1.9353432760567704e-158
zh	9.370023105245346e-06	1.1171323796607264e-158	3.8578592866830766e-235

==> sections/tables/shift_xnli.tex <==
\begin{table*}[ht]
\centering
\caption{Experiment results of applying mean difference shift to m-BERT on XNLI test-set. Shifting weights are selected according to the best results on XNLI dev-set.}
\label{tab:xnli}
\footnotesize
\setlength\tabcolsep{3pt}
\begin{tabular}{c|cccccccccccc|c}
\toprule
% \hline
& en & de & es & ar & el & fr & hi & ru & th & tr & vi & zh & avg w/o en \\
\midrule
% finetune all layers & 78.88 & 65.39 & 68.88 & 58.86 & 60.16 & 68.44 & 53.13 & 63.83 & 41.22 & 52.87 & 66.41 & 64.61 & 60.35 \\
finetune all layers & 80.86 & 67.05 & 70.6 & 59.94 & 56.67 & 70.42 & 46.65 & 66.97 & 41.70 & 50.10 & 40.68 & 67.20 & 58.00 \\
\midrule
finetune last 6 layers & 82.16 & 69.34 & 74.73 & 63.91 & 61.52 & 72.95 & 51.00 & 69.46 & 48.94 & 57.23 & 40.76 & 69.96 & 61.80 \\
+ MDS & - & \textbf{69.72} & 74.57 & \textbf{64.53} & \textbf{62.02} & 72.42 & \textbf{51.28} & \textbf{69.56} & \textbf{49.90} & \textbf{57.45} & \textbf{43.07} & \textbf{70.16} & \textbf{62.24} \\
% + mean difference shift & - & \textbf{69.82} & 74.73 & \textbf{64.71} & \textbf{62.23} & 72.95 & \textbf{51.28} & \textbf{69.56} & \textbf{49.90} & \textbf{57.47} & \textbf{43.07} & \textbf{70.16} & \textbf{62.35} \\
\midrule
% best shifting weight &   & 0.9 & 0.0 & 0.8 & 1.0 & 0.0 & 0.3 & 0.3 & 0.4 & 0.1 & 0.5 & 2.0 & \\
shifting weight &   & 1.5 & 0.2 & 1.0 & 0.9 & 0.7 & 0.3 & 1.0 & 0.4 & 0.4 & 0.5 & 2.0 \\
\bottomrule
\end{tabular}
\vspace{-0.25cm}
\end{table*}

==> sections/tables/word_retrieval.tex <==
\begin{table*}[t!]
\caption{The result of contexualized word retrieval with the 11th layer BERT representations.}
\label{tab:word}
\centering
\footnotesize
\setlength\tabcolsep{3pt}
\begin{tabular}{l|ccccccccccc}
\toprule
Method &de	&es	&ar	&el	&fr	&hi	&ru	&vi 	&th	&tr	&zh\\ \midrule
Original &0.00065	&0.00146	&0.00042	&0.00078	&0.00162	&0.00039	&0.00060	&0.00112	&0.00087	&0.00091	&0.00045\\	
MDS	    &0.00077	&0.00156	&0.00060	&0.00119	&0.00173	&0.00056	&0.00072	&0.00124	&0.00110	&0.00102	&0.00052\\
MUSE    &0.00046   &0.00128   &0.00027   &0.00036   &0.00144   &0.00026   &0.00042   &0.00084   &0.00063	&0.00072	&0.00022\\
Zero mean   &\bf{0.00171}	&\bf{0.00237}	&\bf{0.00153}	&\bf{0.00354}	&\bf{0.00266}	&\bf{0.00183}	&\bf{0.00200}	&\bf{0.00286} &\bf{0.00207}	&\bf{0.00243}	&\bf{0.00153}\\
\bottomrule
\end{tabular}
\end{table*}

==> sections/trans-orig.tex <==

\section{Unsupervised Token Translation} 
In this section, we showed that the implicit language-specific information in
the embedding space could be disentangled from semantic embeddings. 
We used MDS to make m-BERT take a sentence in $L_1$ as input, and
\textit{translate} it into a sentence in $L_2$.


\subsection{Setup}

The formulation of MDS was modified slightly from (\ref{eq:MDS}):
$\tilde{\vect{h}}^l_{x_i} = \vect{h}^l_{x_i} +
\alpha\left(\vect{R}^l_{L_2}-\vect{R}^l_{L_1}\right)$, where $\alpha$ was a
hyperparameter, and we will see its influence later in the experimental
results.
Given the input, the token embeddings were modified at a specific layer $l$. 
The $l+1$-th layer took the modified embeddings as input, and the final layer
generated a sequence of tokens. 
The sentences in this experiment were from XNLI test-set, which contains 15
languages, including low resource languages such as Swahili and Urdu. 

\subsection{Evaluation metrics}

We use two different metrics to analyze the results of unsupervised token
translation quantitatively. 
\paragraph{BLEU-1 score} This metric measures the translation quality without
considering the fluency of the converted sequence.

\paragraph{Convert Rate}
Besides translation quality, we also calculated convert rate, the percentage of
tokens converted from source language to target language, which was defined as
follow:
\[ \text{convert rate} = \frac{\text{\# of } y \in (V_t-V_s)}{\text{\# of } y - \text{\# of } y \in V_s\cap V_t},\]
where $y$ is the output tokens of the model, $V_s, V_t$ is the token set of the
source and target language. 
Shared tokens in both vocabularies were not taken into account therefore
excluded from the numerator and denominator term.

\subsection{Results}
Surprisingly, we were able to get predicted tokens in language $L_2$ from $L_1$
input by applying MDS, and many of the predicted tokens were the token-level
translation of the input tokens in $L_1$, even on the low resource languages.
The sample outputs were shown in Appendix~\ref{sec:appendix}.

\input{sections/tables/translations}


Table~\ref{tab:mt} shows the quantitative results. First, although the
translation results were not comparable to the existing unsupervised
translation methods~\citep{kim2018improving}, it showed strong evidence that we
could manipulate the language-specific information in the token embedding space
by MDS, and force m-BERT to switch from one language to another. 
Second, we observed that as $\alpha$ became larger, the model converted more
tokens to target language $L_2$ and never decoded tokens not belonging to $L_1$
and $L_2$. When given a negative $\alpha$, the model always decoded tokens
belonging to $L_1$. 
The above observation showed that in the embedding space, the direction related
to language is unique. 
We showed a further analysis of $\alpha$ in Appendix~\ref{sec:appendix}.


% The covert rate shows that most of the tokens can be converted into another language. The BLEU-1 scores also show that many of the converted tokens are their translated words without considering the fluency of the converted sequence.


==> sections/zeroshot-orig.tex <==
\section{Cross-Lingual Transfer}

\subsection{Setup}
In zero-shot cross-lingual transfer learning, m-BERT was fine-tuned on the
source language, which was English in the following experiments, and tested on
languages never seen during fine-tuning.
For each language, we had around 5M tokens from Wikipedia documents to compute
the language representations.

\paragraph{Zero-mean} 
During fine-tuning, we applied Zero-mean on the token embeddings of the source
language and forwarding the modified embeddings to the remaining layers during
training. 
While testing, we fed the fine-tuned model with target language data and
applied Zero-mean to the embeddings at layer $l$ as well. 
The means of language vectors were extracted from the Wikipedia data from the
\textbf{pre-trained} model.

\paragraph{MDS} 
In this approach, we did not need to modify embeddings when training. 
While testing, we applied MDS to the embeddings at layer $l$. 
The mean difference vectors were extracted from Wikipedia data by
\textbf{fine-tuned} model.

\subsection{Tasks}
We did the experiments on two tasks, Part-of-Speech (POS) Tagging and
Dependency Parsing, to show that our methods could improve cross-lingual
zero-shot learning performance.

\paragraph{Part-of-Speech Tagging} For POS tagging, we used the Universal
Dependencies v2.5~\citep{udpos} treebanks for 
90 languages. Each word was assigned one of 17 universal
POS tags. 
The model was trained on English and tested on 13 other languages. 

\paragraph{Dependency Parsing} For dependency parsing, we used languages with
nonzero amount of training data in CoNLL 2018 Shared
Task~\citep{zeman-etal-2018-conll}. We evaluated the zero-shot performance on 6
low-resource languages that do not have an official development set. Note that
most of the testing languages in dependency parsing had not been included in
the pretrained languages of
m-BERT\footnote{https://github.com/google-research/bert/blob/master/multilingual.md}
except for Kazakh and Irish. 



\subsection{Results}

Table~\ref{tab:pos} and Table~\ref{tab:dep} compared the results of baselines
and our methods on POS tagging and dependency parsing, respectively. 
For the POS tagging task, Zero-mean and MDS both improved the performances on
the testing sets across languages with only a few exceptions.
MDS was not helpful in Thai (th), while both approaches did not improve on
Vietnamese (vi).
For dependency parsing, although most of the testing languages were not in the
pretrained languages of m-BERT, zero-shot transfer learning still achieved
reasonable performance.
We observed that although Zero-mean does not improve the performance in
dependency parsing, MDS improved the performance except for Irish, which showed
the effectiveness of MDS. 

% \subsection{Training Details}

% \paragraph{Cross-lingual NLI}
% Cross-lingual Natural Language Inference(XNLI)~\citep{conneau:18} contains 5,000 test and 2,500 dev pairs. The pairs are annotated with entails, contradicts, or neutral. English data is translated to 14 other languages by professional translators and used for evaluation.


% In previous works~\citep{pires2019multilingual, conneau2019cross}, people attempted to solve cross-lingual transfer tasks like XNLI in a purely zero-shot setting by training on English dataset and then testing on the dataset of other languages. 
% However, as we have shown, the representation has language-specific information, so the training language and the testing languages still have mismatched representations. 
% We tried to eliminate the difference in language-specific information using MDS. 

% For the XNLI task, we finetuned the m-BERT model on the English dataset while fixing the first six layers of it, as the transfer results of finetuning the last 6 layers are slightly better than finetuning the whole BERT model. 

% The results show  MDS on the XNLI dataset, the language-specific information can be eliminated to some extent, and the modified representations can preserve more semantic information instead of mixed with language-specific information. 

% As for Spanish (es) and French (fr), MDS did not bring any advantages. We speculated that the results came from the higher subword overlapping with English. Some shared subwords do not have the same meaning in English and the target language.

% Because MDS used one mean vector to present language-specific representation without considering the difference among vocabularies, simply apply MDS to all vocabularies of these languages may hurt performance instead. A more delicate mechanism should be considered to apply different shifts for different vocabularies. We leave this research topic for future work.


